Dipping PLMs Sauce: Bridging Structure and Text for Effective Knowledge Graph Completion via Conditional Soft Prompting

Knowledge Graph Completion (KGC) often requires both KG structural and textual information to be effective. Pre-trained Language Models (PLMs) have been used to learn the textual information, usually under the fine-tune paradigm for the KGC task. However, the fine-tuned PLMs often overwhelmingly focus on the textual information and overlook structural knowledge. To tackle this issue, this paper proposes CSProm-KG (Conditional Soft Prompts for KGC) which maintains a balance between structural information and textual knowledge. CSProm-KG only tunes the parameters of Conditional Soft Prompts that are generated by the entities and relations representations. We verify the effectiveness of CSProm-KG on three popular static KGC benchmarks WN18RR, FB15K-237 and Wikidata5M, and two temporal KGC benchmarks ICEWS14 and ICEWS05-15. CSProm-KG outperforms competitive baseline models and sets new state-of-the-art on these benchmarks. We conduct further analysis to show (i) the effectiveness of our proposed components, (ii) the efficiency of CSProm-KG, and (iii) the flexibility of CSProm-KG.

==> tables/head_variants.tex <==
\begin{table}[!htbp]
	\centering
	\begin{small}
	\resizebox{0.9\columnwidth}{!}{
	\begin{tabular}{lllll}
		\toprule
        Methods &MRR &H@1 &H@3 &H@10 \\
		\midrule\midrule
		w/ head &.538 &.495 &.556 &.622  \\
		w/o head  &.514 &.472 &.531 &.596 \\
\bottomrule
\addlinespace
\end{tabular}
}
\caption{Ablation study of \method with or without heads (ConvE). The results are obtained on \datawnrr.  }
\label{tab:head variants} 
\end{small}
\end{table}

==> tables/model_focus.tex <==
\begin{table}[!htbp]
	\centering
	\begin{small}
	\resizebox{\columnwidth}{!}{
    	\begin{tabular}{lccccccccc}
    		\toprule  
    		 &MRR &H@1 &H@3 &H@10 \\
    		\midrule
            prompt \method &.538 &.495 &.556 &.622 \\
            finetune \method &.408 &.386 &.419 & .443 \\
            \midrule
            freeze 13-24 layers &.427 &.406 &.436 &.468 \\
            freeze 1-12 layers &.411 &.389 &.421 &.448 \\
            \midrule
            freeze 2-24 layers &.404 &.388 &.412 &.430 \\
            freeze 1-23 layers &.505 &.472 &.517 &.568 \\
            \bottomrule
            \addlinespace
        \end{tabular}
    }
    \end{small}\label{tab:model focus}
    \caption{Ablation study of fine-tuning variants}
\end{table}

==> tables/soft_prompt_variants.tex <==
\begin{table}[!htbp]
	\centering
	\begin{small}
	\resizebox{0.9\columnwidth}{!}{
	\begin{tabular}{lllll}
		\toprule
        Methods &MRR &H@1 &H@3 &H@10 \\
		\midrule\midrule
		layer-wise &- &- &- &-  \\
		non-layer-wise  &- &- &- &- \\
\bottomrule
\addlinespace
\end{tabular}
}
\caption{Ablation study of \method with layer-wise or non-layer-wise soft prompt. The results are obtained on \datawnrr }
\label{tab:soft prompt variants} 
\end{small}
\end{table}

==> tables/structure_variants.tex <==
\begin{table}[!htbp]
	\centering
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{llllll}
		\toprule
        Dataset &Variants &MRR &H@1 &H@3 &H@10 \\
		\midrule\midrule
        \multirow{2}{*}{\datawnrr} &Joint&.563 &.413 &.585 &.660 \\
        &Separated&.519 &.469 &.532 &.621 \\
        \midrule
        \multirow{2}{*}{\datafb} &Joint&.354 &.263  &.388 &.536 \\
        &Separated&.344 &.254 &.376 &.524 \\
\bottomrule
\addlinespace
\end{tabular}
}
\caption{Result of \method structure variants on \datawnrr and \datafb}
\label{tab:sturcture variants} 
\end{table}
